Efficient coding of 360{\deg} videos exploiting inactive regions in projection formats

This paper presents an efficient method for encoding common projection formats in 360$^\circ$ video coding, in which we exploit inactive regions. These regions are ignored in the reconstruction of the equirectangular format or the viewport in virtual reality applications. As the content of these pixels is irrelevant, we neglect the corresponding pixel values in ratedistortion optimization, residual transformation, as well as inloop filtering and achieve bitrate savings of up to 10%.

==> gfx2/FORPAPER_RDcurve02_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{12.60}{12.60}\selectfont\strut}%
\psfrag{0000000000000}[cl][cl]{\matlabtextA Irrelevant}%
\psfrag{00000000001}[cl][cl]{\matlabtextA Standard}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{15.40}{15.40}\selectfont\strut}%
\psfrag{013}[tc][tc]{\matlabtextB Bitrate}%
\psfrag{014}[bc][bc]{\matlabtextB PSNR, WSPSNR [dB]}%
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{15.40}{15.40}\bfseries\boldmath\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextC AerialCity, CISP, BD-Rate (WSPSNR): -3.0463\%}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextD{\color[rgb]{0.150,0.150,0.150}\fontsize{14.00}{14.00}\selectfont\strut}%
\psfrag{002}[tc][tc]{\matlabtextD $\times10^{5}$}%
%
%% </xscale>
%
%% <xtick>
%
\psfrag{003}[ct][ct]{\matlabtextD $0$}%
\psfrag{004}[ct][ct]{\matlabtextD $5$}%
\psfrag{005}[ct][ct]{\matlabtextD $10$}%
\psfrag{006}[ct][ct]{\matlabtextD $15$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextD $34$}%
\psfrag{008}[rc][rc]{\matlabtextD $36$}%
\psfrag{009}[rc][rc]{\matlabtextD $38$}%
\psfrag{010}[rc][rc]{\matlabtextD $40$}%
\psfrag{011}[rc][rc]{\matlabtextD $42$}%
%
%% </ytick>

==> gfx2/FORPAPER_RDcurve_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{12.60}{12.60}\selectfont\strut}%
\psfrag{000000000000000000000000000000}[cl][cl]{\matlabtextA Irrelevant encoding, WSPSNR}%
\psfrag{0000000000000000000000000001}[cl][cl]{\matlabtextA Standard Encoding, WSPSNR}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{15.40}{15.40}\selectfont\strut}%
\psfrag{013}[tc][tc]{\matlabtextB Bitrate}%
\psfrag{014}[bc][bc]{\matlabtextB PSNR, WSPSNR [dB]}%
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{15.40}{15.40}\bfseries\boldmath\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextC AerialCity, CISP, BD-Rate (WSPSNR): -3.0463\%}%
%
%% </text>
%
%% <xscale>
%
\providecommand\matlabtextD{\color[rgb]{0.150,0.150,0.150}\fontsize{14.00}{14.00}\selectfont\strut}%
\psfrag{002}[tc][tc]{\matlabtextD $\times10^{5}$}%
%
%% </xscale>
%
%% <xtick>
%
\psfrag{003}[ct][ct]{\matlabtextD $0$}%
\psfrag{004}[ct][ct]{\matlabtextD $5$}%
\psfrag{005}[ct][ct]{\matlabtextD $10$}%
\psfrag{006}[ct][ct]{\matlabtextD $15$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextD $34$}%
\psfrag{008}[rc][rc]{\matlabtextD $36$}%
\psfrag{009}[rc][rc]{\matlabtextD $38$}%
\psfrag{010}[rc][rc]{\matlabtextD $40$}%
\psfrag{011}[rc][rc]{\matlabtextD $42$}%
%
%% </ytick>

==> gfx2/TMPresult_OHP_AerialCity_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{12.60}{12.60}\selectfont\strut}%
\psfrag{0000000000000}[cl][cl]{\matlabtextA data1ddddd}%
\psfrag{00000001}[cl][cl]{\matlabtextA data2}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{15.40}{15.40}\selectfont\strut}%
\psfrag{010}[tc][tc]{\matlabtextB Bitrate}%
\psfrag{011}[bc][bc]{\matlabtextB PSNR, WSPSNR [dB]}%
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{15.40}{15.40}\bfseries\boldmath\selectfont\strut}%
\psfrag{009}[bc][bc]{\matlabtextC AerialCity, OHP, BD-Rate (WSPSNR): -9.7735\%}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextD{\color[rgb]{0.150,0.150,0.150}\fontsize{14.00}{14.00}\selectfont\strut}%
\psfrag{002}[ct][ct]{\matlabtextD $0$}%
\psfrag{003}[ct][ct]{\matlabtextD $5000$}%
\psfrag{004}[ct][ct]{\matlabtextD $10000$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextD $34$}%
\psfrag{006}[rc][rc]{\matlabtextD $36$}%
\psfrag{007}[rc][rc]{\matlabtextD $38$}%
\psfrag{008}[rc][rc]{\matlabtextD $40$}%
%
%% </ytick>
